Harnessing Hard Mixed Samples with Decoupled Regularizer

Mixup is an efficient data augmentation approach that improves the generalization of neural networks by smoothing the decision boundary with mixed data. Recently, dynamic mixup methods have improved previous static policies effectively (e.g., linear interpolation) by maximizing target-related salient regions in mixed samples, but excessive additional time costs are not acceptable. These additional computational overheads mainly come from optimizing the mixed samples according to the mixed labels. However, we found that the extra optimizing step may be redundant because label-mismatched mixed samples are informative hard mixed samples for deep models to localize discriminative features. In this paper, we thus are not trying to propose a more complicated dynamic mixup policy but rather an efficient mixup objective function with a decoupled regularizer named Decoupled Mixup (DM). The primary effect is that DM can adaptively utilize those hard mixed samples to mine discriminative features without losing the original smoothness of mixup. As a result, DM enables static mixup methods to achieve comparable or even exceed the performance of dynamic methods without any extra computation. This also leads to an interesting objective design problem for mixup training that we need to focus on both smoothing the decision boundaries and identifying discriminative features. Extensive experiments on supervised and semi-supervised learning benchmarks across seven datasets validate the effectiveness of DM as a plug-and-play module. Source code and models are available at https://github.com/Westlake-AI/openmixup

==> Tabs/sl_imagenet_deit.tex <==
\begin{table}[H]
\centering
    \setlength{\tabcolsep}{1.0mm}
    \caption{Top-1 Acc (\%)$\uparrow$ of classification on ImageNet-1k based on DeiT-S.}
    \vspace{-4pt}
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
    Methods         & MCE   & \bf{MD(CE)} \\ \hline
    vanilla         & 78.60 & -           \\
    DeiT            & 79.80 & \bf{80.37}  \\
    Mixup           & 79.65 & \bf{80.04}  \\
    CutMix          & 79.78 & \bf{80.20}  \\
    SaliencyMix     & 79.32 & \bf{79.86}  \\
    PuzzleMix       & 79.84 & \bf{80.25}  \\
    ResizeMix$^*$   & 79.41 & \bf{79.89}  \\
    ResizeMix$^*$   & 79.93 & \bf{80.02}  \\
    TransMix$^\dag$ & 80.70 & -           \\
    AutoMix$^*$     & 80.75 & \bf{80.91}  \\
    SAMix$^*$       & 80.94 & \bf{81.12}  \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:sl_imagenet_deit}
\end{table}


==> Tabs/ssl_cifar10.tex <==
\begin{table}[b]
    \vspace{-1.5em}
    \centering
    \setlength{\tabcolsep}{1.2mm}
\caption{
    Top-1 Acc (\%)$\uparrow$ of semi-supervised learning on CIFAR-10 (using 250 and 4000 labels) based on WRN-28-2. Notice that DM denotes using DM(CE) and AS, Con denotes various unsupervised consistency losses, Rot denotes the rotation loss in ReMixMatch, and CPL denotes the curriculum labeling in FlexMatch.}
\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{ll|cc}
    \toprule
                  Methods          & Losses     & 250                        & 4000                       \\ \hline
                  Pseudo-Labeling  & CE         & 53.51{\scr $\pm$2.20}      & 84.92{\scr $\pm$0.19}      \\
\rowcolor{gray94} MixMatch         & CE+Con     & 86.37{\scr $\pm$0.59}      & 93.34{\scr $\pm$0.26}      \\
                  ReMixMatch       & CE+Con+Rot & 93.70{\scr $\pm$0.05}      & 95.16{\scr $\pm$0.01}      \\
\rowcolor{gray85} \bf{MixMatch+DM} & CE+Con+DM  & 89.16{\scr $\pm$0.71}      & 95.15{\scr $\pm$0.68}      \\
                  UDA              & CE+Con     & 94.84{\scr $\pm$0.06}      & 95.71{\scr $\pm$0.07}      \\
\rowcolor{gray94} FixMatch         & CE+Con     & 95.14{\scr $\pm$0.05}      & 95.79{\scr $\pm$0.08}      \\
                  FlexMatch        & CE+Con+CPL & 95.02{\scr $\pm$0.09}      & 95.81{\scr $\pm$0.01}      \\
\rowcolor{gray94} FixMatch+Mixup   & CE+Con+MCE & 95.05{\scr $\pm$0.23}      & 95.83{\scr $\pm$0.19}      \\
\rowcolor{gray85} \bf{FixMatch+DM} & CE+Con+DM  & \bf{95.23{\scr $\pm$0.09}} & \bf{95.87{\scr $\pm$0.11}} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ssl_cifar10}
    \vspace{-0.5em}
\end{table}

